Training Variational Autoencoders with Buffered Stochastic Variational Inference

The recognition network in deep latent variable models such as variational autoencoders (VAEs) relies on amortized inference for efficient posterior approximation that can scale up to large datasets. However, this technique has also been demonstrated to select suboptimal variational parameters, often resulting in considerable additional error called the amortization gap. To close the amortization gap and improve the training of the generative model, recent works have introduced an additional refinement step that applies stochastic variational inference (SVI) to improve upon the variational parameters returned by the amortized inference model. In this paper, we propose the Buffered Stochastic Variational Inference (BSVI), a new refinement procedure that makes use of SVI's sequence of intermediate variational proposal distributions and their corresponding importance weights to construct a new generalized importance-weighted lower bound. We demonstrate empirically that training the variational autoencoders with BSVI consistently out-performs SVI, yielding an improved training procedure for VAEs.

==> figures/compare_buff_diff.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{images/compare_buff_diff_1.pdf}
\caption{TODO (Jay): Update the caption}
\label{fig:compare_buff_diff}
\end{figure}

==> figures/compare_kl.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{images/compare_kl.pdf}
\caption{TODO (Jay): Update the caption}
\label{fig:compare_kl}
\end{figure}

==> figures/compare_pi.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{images/compare_pi.pdf}
\caption{Plot of the weighted mean $\cfrac{1}{k}\sum\limits_{i=0}^{k} i \pi_i$ of the buffer weight during training. Higher values imply that the model is benefiting from SVI.}
\label{fig:compare_pi}
\end{figure}

==> figures/compare_svi_diff.tex <==
\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{images/compare_svi_diff.pdf}
\caption{TODO}
\jw{Not sure what to call this quantity (svi-diff).}
\label{fig:compare_svi_diff}
\end{figure}

==> figures/speed.tex <==
\begin{figure}[h]
\vspace{.3in}
\centerline{\fbox{This figure intentionally left non-blank}}
\vspace{.3in}
\caption{Show computational graph visualization?}
\end{figure}

==> figures/training_metrics_wide.tex <==
\begin{figure*}[!ht]
\centering
\begin{subfigure}[b]{\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{images/compare_svi_diff_wide.pdf}
\caption{Difference between lower bounds achieved by $q_k$ (SVI-$k$) and $q_0$ (SVI-$0$) during training.}
\label{fig:compare_svi_diff}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{images/compare_buff_diff_1_wide.pdf}
\caption{Difference between the BSVI-$k$ bound and SVI-$k$ bound during training.}
\label{fig:compare_buff_diff}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{images/compare_pi_wide.pdf}
\caption{Plot of the buffer weight average (defined as $\Expect_{\pi(i)} i / k$) during training when the buffer weight is optimized.}
\label{fig:compare_pi}
\end{subfigure}

% \begin{subfigure}[b]{\columnwidth}
% \centering
% \includegraphics[width=\columnwidth]{images/compare_kl.pdf}
% \caption{TODO: KL}
% \label{fig:compare_kl}
% \end{subfigure}

\caption{Plots of metrics during BSVI-$k$ training, where $k = 9$. Since BSVI-$k$ uses SVI-$k$ as a subroutine, it is easy to check how the BSVI-$k$ bound compares against the SVI-$k$ and the amortized ELBO (SVI-$0$) bounds on a random mini-batch at every iteration during training.}
\end{figure*}

==> tables/fmnist_train.tex <==
\begin{table*}[!h]
\centering
\caption{Training set performance on the FashionMNIST dataset. Comparison between VAE, IWAE with $k'=10$ particles, SVI with $k'=10$ SVI steps, and BSVI with $k = 9$ SVI steps.}
\label{table:fmnist_train}
\begin{center}
\begin{tabular}{l|c|ccc}
\textbf{Model} & \textbf{Log-likelihood} & \textbf{ELBO*} & \textbf{KL*} & \textbf{Reconstruction*} \\
\hline
VAE                & -1686.11 $\pm$ 2.40 & -1688.84 $\pm$ 2.27 & 11.34 $\pm$ 1.01 & 1677.50 $\pm$ 3.16 \\
IWAE-$k'$          & -1659.12 $\pm$ 0.59 & -1663.80 $\pm$ 0.53 & 33.62 $\pm$ 0.31 & 1630.18 $\pm$ 0.56 \\
SVI-$k'$           & -1666.89 $\pm$ 2.47 & -1675.15 $\pm$ 2.11 & 25.34 $\pm$ 1.80 & 1649.81 $\pm$ 3.90 \\
BSVI-$k$-SIR       & -1653.34 $\pm$ 1.36 & -1660.79 $\pm$ 1.35 & 41.91 $\pm$ 0.15 & 1618.88 $\pm$ 1.51 \\
BSVI-$k$-DS        & -1653.47 $\pm$ 0.85 & -1661.15 $\pm$ 0.82 & \textbf{42.13 $\pm$ 0.23} & 1619.02 $\pm$ 1.05 \\
BSVI-$k$           & \textbf{-1652.87 $\pm$ 0.87} & \textbf{-1660.27 $\pm$ 0.89} & 41.85 $\pm$ 0.12 & \textbf{1618.43 $\pm$ 0.86} \\
BSVI-$k$-$\pi$     & -1654.35 $\pm$ 0.74 & -1661.99 $\pm$ 0.68 & 42.00 $\pm$ 0.48 & 1619.99 $\pm$ 1.09 \\
BSVI-$k$-SIR-$\pi$ & -1654.75 $\pm$ 1.19 & -1662.18 $\pm$ 1.25 & 41.58 $\pm$ 0.22 & 1620.60 $\pm$ 1.44 \\
\end{tabular}
% \begin{tabular}{lccccc}
% \textbf{Model} & \textbf{Log-likelihood} & \textbf{ELBO} & \textbf{ELBO*} & \textbf{KL*} & \textbf{Reconstruction*} \\
% \hline
% VAE & -1686.11 $\pm$ 2.40 & -1690.66 $\pm$ 2.21 & -1688.84 $\pm$ 2.27 & 11.34 $\pm$ 1.01 & 1677.50 $\pm$ 3.16 \\
% IWAE-$k'$ & -1659.12 $\pm$ 0.59 & -1691.95 $\pm$ 0.65 & -1663.80 $\pm$ 0.53 & 33.62 $\pm$ 0.31 & 1630.18 $\pm$ 0.56 \\
% SVI-$k'$ & -1666.89 $\pm$ 2.47 & \textbf{-1687.38 $\pm$ 1.59} & -1675.15 $\pm$ 2.11 & 25.34 $\pm$ 1.80 & 1649.81 $\pm$ 3.90 \\
% BSVI-$k$-DS & -1653.47 $\pm$ 0.85 & -1694.63 $\pm$ 0.32 & -1661.15 $\pm$ 0.82 & \textbf{42.13 $\pm$ 0.23} & 1619.02 $\pm$ 1.05 \\
% BSVI-$k$ & \textbf{-1652.87 $\pm$ 0.87} & -1693.86 $\pm$ 0.77 & \textbf{-1660.27 $\pm$ 0.89} & 41.85 $\pm$ 0.12 & \textbf{1618.43 $\pm$ 0.86} \\
% BSVI-$k$-$\pi$ & -1654.35 $\pm$ 0.74 & -1695.55 $\pm$ 0.41 & -1661.99 $\pm$ 0.68 & 42.00 $\pm$ 0.48 & 1619.99 $\pm$ 1.09 \\
% BSVI-$k$-SIR & -1653.34 $\pm$ 1.36 & -1694.32 $\pm$ 0.72 & -1660.79 $\pm$ 1.35 & 41.91 $\pm$ 0.15 & 1618.88 $\pm$ 1.51 \\
% BSVI-$k$-SIR-$\pi$ & -1654.75 $\pm$ 1.19 & -1695.27 $\pm$ 0.66 & -1662.18 $\pm$ 1.25 & 41.58 $\pm$ 0.22 & 1620.60 $\pm$ 1.44 \\
% \end{tabular}
\end{center}
\end{table*}


==> tables/omni_train.tex <==
\begin{table*}[!h]
\centering
\caption{\rs{TODO: Modify these tables to new format.} Training set performance on the Omniglot dataset. Comparison between VAE, IWAE with $k'=10$ particles, SVI with $k'=10$ SVI steps, and BSVI with $k = 9$ SVI steps.} \label{table:omni_train}
\begin{center}
\begin{tabular}{l|c|ccc}
\textbf{Model} & \textbf{Log-likelihood} & \textbf{ELBO*} & \textbf{KL*} & \textbf{Reconstruction*} \\
\hline
VAE                & -88.60 $\pm$ 0.18 & -88.66 $\pm$ 0.18 & 1.00 $\pm$ 0.13 & 87.66 $\pm$ 0.19 \\
IWAE-$k'$          & -87.09 $\pm$ 0.12 & \textbf{-87.88 $\pm$ 0.12} & 4.18 $\pm$ 0.19 & 83.70 $\pm$ 0.29 \\
SVI-$k'$           & -88.09 $\pm$ 0.16 & -88.18 $\pm$ 0.15 & 1.38 $\pm$ 0.14 & 86.80 $\pm$ 0.27 \\
BSVI-$k$-SIR       & -87.24 $\pm$ 0.22 & -88.57 $\pm$ 0.25 & 7.67 $\pm$ 0.22 & 80.89 $\pm$ 0.44 \\
BSVI-$k$-DS        & \textbf{-87.00 $\pm$ 0.11}& -88.13 $\pm$ 0.10 & 8.30 $\pm$ 0.18 & 79.83 $\pm$ 0.23 \\
BSVI-$k$           & -87.11 $\pm$ 0.11 & -88.23 $\pm$ 0.10 & 8.45 $\pm$ 0.22 & 79.77 $\pm$ 0.28 \\
BSVI-$k$-$\pi$     & -87.10 $\pm$ 0.11 & -88.24 $\pm$ 0.10 & \textbf{8.67 $\pm$ 0.27} & \textbf{79.57 $\pm$ 0.31} \\
BSVI-$k$-SIR-$\pi$ & -87.17 $\pm$ 0.10 & -88.45 $\pm$ 0.11 & 7.63 $\pm$ 0.04 & 80.83 $\pm$ 0.13 \\
\end{tabular}
% \begin{tabular}{lccccc}
% \textbf{Model} & \textbf{Log-likelihood} & \textbf{ELBO} & \textbf{ELBO*} & \textbf{KL*} & \textbf{Reconstruction*} \\
% \hline
% VAE         & -88.60 $\pm$ 0.18 & -88.71 $\pm$ 0.18 & -88.66 $\pm$ 0.18 & 1.00 $\pm$ 0.13 & 87.66 $\pm$ 0.19 \\
% IWAE-$k'$        & -87.09 $\pm$ 0.12 & -88.97 $\pm$ 0.03 & \textbf{-87.88 $\pm$ 0.12} & 4.18 $\pm$ 0.19 & 83.70 $\pm$ 0.29 \\
% SVI-$k'$         & -88.09 $\pm$ 0.16 & \textbf{-88.38 $\pm$ 0.13} & -88.18 $\pm$ 0.15 & 1.38 $\pm$ 0.14 & 86.80 $\pm$ 0.27 \\
% BSVI-$k$-DS   & \textbf{-87.00 $\pm$ 0.11} & -89.32 $\pm$ 0.11 & -88.13 $\pm$ 0.10 & 8.30 $\pm$ 0.18 & 79.83 $\pm$ 0.23 \\
% BSVI-$k$        & -87.11 $\pm$ 0.11 & -89.47 $\pm$ 0.10 & -88.23 $\pm$ 0.10 & 8.45 $\pm$ 0.22 & 79.77 $\pm$ 0.28 \\
% BSVI-$k$-SIR    & -87.24 $\pm$ 0.22 & -89.62 $\pm$ 0.21 & -88.57 $\pm$ 0.25 & 7.67 $\pm$ 0.22 & 80.89 $\pm$ 0.44 \\
% BSVI-$k$-$\pi$     & -87.10 $\pm$ 0.11 & -89.49 $\pm$ 0.10 & -88.24 $\pm$ 0.10 & \textbf{8.67 $\pm$ 0.27} & \textbf{79.57 $\pm$ 0.31} \\
% BSVI-$k$-SIR-$\pi$ & -87.17 $\pm$ 0.10 & -89.48 $\pm$ 0.09 & -88.45 $\pm$ 0.11 & 7.63 $\pm$ 0.04 & 80.83 $\pm$ 0.13 \\
% \end{tabular}
\end{center}
\end{table*}


==> tables/svhn_train.tex <==
\begin{table*}[!h]
\centering
\caption{Training set performance on the grayscale SVHN dataset. Comparison between VAE, IWAE with $k'=10$ particles, SVI with $k'=10$ SVI steps, and BSVI with $k = 9$ SVI steps.} 
\label{table:svhn_train}
\begin{center}
\begin{tabular}{l|c|ccc}
\textbf{Model} & \textbf{Log-likelihood} & \textbf{ELBO*} & \textbf{KL*} & \textbf{Reconstruction*} \\
\hline
VAE                & -2384 $\pm$ 13.58 & -2384 $\pm$ 13.59 & 0.5 $\pm$ 0.09 & 2384 $\pm$ 13.58 \\
IWAE-$k'$          & -2345 $\pm$ 8.77  & -2350 $\pm$ 9.58 & 2.19 $\pm$ 0.03 & 2348 $\pm$ 9.55 \\
SVI-$k'$           & -2274 $\pm$ 8.87  & -2280 $\pm$ 8.34 & 56 $\pm$ 5.75 & 2224 $\pm$ 12.20 \\
BSVI-$k$-SIR       & -2260 $\pm$ 2.73    & -2268 $\pm$ 3.01 & 62.17 $\pm$ 5.51 & 2206 $\pm$ 4.86 \\
BSVI-$k$-DS        & \textbf{-2255.28 $\pm$ 7.38} & \textbf{-2262 $\pm$ 7.51} & 59 $\pm$ 5.34 & 2203 $\pm$ 9.28 \\
BSVI-$k$           & -2255.47 $\pm$ 7.31 & -2263 $\pm$ 7.47 & \textbf{62.20 $\pm$ 4.27} & \textbf{2201 $\pm$ 8.26} \\
BSVI-$k$-$\pi$     & -2261 $\pm$ 5.09    & -2268 $\pm$ 6.13 & 58 $\pm$ 5.10 & 2210 $\pm$ 1.43 \\
BSVI-$k$-SIR-$\pi$ & -2258 $\pm$ 3.89    & -2265 $\pm$ 3.30 & 60 $\pm$ 6.36 & 2206 $\pm$ 7.79 \\
\end{tabular}
% \begin{tabular}{lccccc}
% \textbf{Model} & \textbf{Log-likelihood} & \textbf{ELBO} & \textbf{ELBO*} & \textbf{KL*} & \textbf{Reconstruction*} \\
% \hline
% VAE                & -2384 $\pm$ 13.58 & -2385 $\pm$ 13.59 & -2384 $\pm$ 13.59 & 0.5 $\pm$ 0.09 & 2384 $\pm$ 13.58 \\
% IWAE-$k'$          & -2345 $\pm$ 8.77 & -2360 $\pm$ 9.68 & -2350 $\pm$ 9.58 & 2.19 $\pm$ 0.03 & 2348 $\pm$ 9.55 \\
% SVI-$k'$           & -2274 $\pm$ 8.87 & -2318 $\pm$ 6.82 & -2280 $\pm$ 8.34 & 56 $\pm$ 5.75 & 2224 $\pm$ 12.20 \\
% BSVI-$k$-DS        & \textbf{-2255.28 $\pm$ 7.38} & \textbf{-2302 $\pm$ 9.93} & \textbf{-2262 $\pm$ 7.51} & 59 $\pm$ 5.34 & 2203 $\pm$ 9.28 \\
% BSVI-$k$           & -2255.47 $\pm$ 7.31 & -2307 $\pm$ 9.26 & -2263 $\pm$ 7.47 & \textbf{62.20 $\pm$ 4.27} & \textbf{2201 $\pm$ 8.26} \\
% BSVI-$k$-SIR       & -2260 $\pm$ 2.73 & -2312 $\pm$ 7.37 & -2268 $\pm$ 3.01 & 62.17 $\pm$ 5.51 & 2206 $\pm$ 4.86 \\
% BSVI-$k$-$\pi$     & -2261 $\pm$ 5.09 & -2305 $\pm$ 10.83 & -2268 $\pm$ 6.13 & 58 $\pm$ 5.10 & 2210 $\pm$ 1.43 \\
% BSVI-$k$-SIR-$\pi$ & -2258 $\pm$ 3.89 & -2306 $\pm$ 6.56 & -2265 $\pm$ 3.30 & 60 $\pm$ 6.36 & 2206 $\pm$ 7.79 \\
% \end{tabular}
\end{center}
\end{table*}


